Regularity of CR maps into uniformly pseudoconvex hypersurfaces and applications to proper holomorphic maps

We study regularity properties of CR maps in positive codimension valued in pseudoconvex manifolds which carry a nontrivial Levi foliation. We introduce an invariant which can be used to deduce that any sufficiently regular CR map from a minimal manifold into such a foliated target is either generically smooth or geometrically highly constrained, and to show generic smoothness of sufficiently regular CR transversal CR maps between pseudoconvex hypersurfaces. As an application, we discuss boundary regularity of proper holomorphic maps into bounded symmetric domains.

==> abstract.tex <==
\section*{Abstract [EN]}
\small In this thesis, we study the smooth regularity of CR maps between CR submanifolds with targets that are foliated by complex manifolds. As an application, we consider CR-transver\-sal CR maps from strongly pseudoconvex real hypersurfaces into the smooth part of the boundary of classical symmetric domains. For the first, second and third series of classical symmetric domains, we find sharp conditions on the CR-dimension of the source manifold which force any such CR map to be $\cinfty$-smooth on a dense open subset of the source, as long as it satisfies an initial regularity condition. For classical symmetric domains of the fourth kind, we prove that any CR map of sufficient initial regularity is either smooth on a dense open subset or locally takes its values in a single complex line.

We begin by briefly introducing the necessary concepts of CR geometry before turning to a theorem of Lamel \& Mir \cite{lamelmir1} which serves as the main instrument to establish regularity of CR maps. Subsequently, a setup for the analysis of CR maps into pseudoconvex hypersurfaces foliated by complex manifolds is developed and applied to CR maps into boundaries of classical symmetric domains.

\section*{Abstract}
In dieser Arbeit untersuchen wir die $\cinfty$-Regularität von CR-Abbildungen zwischen CR-Teilmannigfaltigkeiten, deren Zielmannigfaltigkeit mit komplexen Mannigfaltigkeiten foliert ist. Als Anwendungsbeispiel konzentrieren wir uns auf CR-transversale CR-Abbildungen, die eine stark pseudokonvexe reelle Hyperfläche in den glatten Teil des Randes eines klassischen symmetrischen Gebiets abbilden. Für die erste, zweite und dritte Reihe klassischer symmetrischer Gebiete finden wir scharfe Bedingungen an die CR-Dimension der Ursprungsmannigfaltigkeit, unter welchen eine solche CR-Abbildung bereits glatt ist, solange sie genügend viele Ableitungen besitzt. Für die klassischen symmetrischen Gebiete vom Typ Vier zeigen wir, dass jede genügend oft differenzierbare CR-Abbildung entweder glatt auf einer dichten offenen Teilmenge ist, oder lokal ihre Werte in einer einzigen komplexen Gerade annimmt.

Wir beginnen mit einer kurzen Einführung in die notwendigen Grundbegriffe der CR-Geometrie, und wenden uns dann einem Satz von Lamel \& Mir \cite{lamelmir1} zu, der das Haupt\-werkzeug für die Regularitätsbeweise bereitstellt. Danach untersuchen wir Abbildungen in pseudokonvexe, mit komplexen Mannigfaltigkeiten folierte Hyperflächen. Zuletzt wenden wir die entwickelten Methoden auf Abbildungen in den Rand klassischer symmetrischer Gebiete an.
\normalsize
